DPSyn: Experiences in the NIST Differential Privacy Data Synthesis Challenges

We summarize the experience of participating in two differential privacy competitions organized by the National Institute of Standards and Technology (NIST). In this paper, we document our experiences in the competition, the approaches we have used, the lessons we have learned, and our call to the research community to further bridge the gap between theory and practice in DP research.

==> primitive_exp.tex <==

\subsection{Exponential Mechanism}
The exponential mechanism (EM)~\cite{focs:mcsherry07} samples from the set of all possible answers according to an exponential distribution, with answers that are ``more accurate'' being sampled with higher probability.  
This approach requires the specification of a quality functions $q$ that takes as input the data $D$, a possible output $o$, and outputs a real-numbered quality score. 
The global sensitivity of the quality functions $\mathsf{GS}_q$ is defined as:
\begin{align}
    \mathsf{GS}_q = \max_{o} \max_{D\simeq D'} |q(D,o) - q_i(D',o)|
    \label{eq:gs_exp}
\end{align} 
The following method $\AA$ satisfies $\epsilon$-differential privacy:
\begin{align}
 \Pr{\AA_q(D)=o} =\frac{ \exp{\left(\frac{\epsilon }{2\,\mathsf{GS}_q}q(D,o)\right)}}{\sum_o' \exp{\left(\frac{\epsilon }{2\,\mathsf{GS}_q}q(D,o')\right)}} \label{eq:exp}
\end{align}

As shown in~\cite{focs:mcsherry07}, if the quality function satisfies the condition that when the input dataset is changed from $D$ to $D'$, the quality scores of all outcomes change in the same direction, i.e., for any neighboring $D$ and $D'$
\[
\left(\exists_o\, q(D,o) \!<\! q(D',o)\right) \!\implies\! \left(\forall_{o'}\,q(D,o') \!\leq \! q(D',o')\right)
\]

Then one can remove the factor of $1/2$ in the exponent of Equation~(\ref{eq:exp}) and return $i$ with probability proportional to $\exp\!{\left(\frac{\epsilon }{\mathsf{GS}_q}q(D,o)\right)}$.  This improves the accuracy of the result.

==> primitive_lap.tex <==

\subsection{Laplace Mechanism}
The Laplace mechanism computes a function $f$ on the input $D$ in a differentially private way, by adding to $f(D)$ a random noise.  The magnitude of the noise depends on $\mathsf{GS}_f$, the \emph{global sensitivity} or the $L_1$ sensitivity of $f$, defined as,
\[
\mathsf{GS}_f = \max\limits_{D\simeq D'} ||f(D) - f(D')||_1
\] 
When $f$ outputs a single element, such a mechanism $\AA$ is given below:
$$
\begin{array}{crl}
& \AA_f(D) & =f(D) + \Lapp{\frac{\mathsf{GS}_f}{\epsilon}}
\end{array}
$$
In the definition above, $\Lapp{\beta}$ denotes a random variable sampled from the Laplace distribution with scale parameter $\beta$ such that $\Pr{\Lapp{\beta}=x} = \frac{1}{2\beta} \myexp{-|x|/\beta}$.  When $f$ outputs a vector, $\AA$ adds independent samples of $\Lapp{\frac{\mathsf{GS}_f}{\epsilon}}$ to each element of the vector.  





==> sec8_related.tex <==

\vspace{-1em}
\section{Related Work}
\label{sec:related}

Differential privacy (DP) has been the \textit{de facto} notion for protecting privacy.
Many DP algorithms have been proposed (see~\cite{dpbook,vadhan2017complexity} for theoretical treatments and~\cite{Li2016book} in a more practical perspective).
Most of the algorithms are proposed for specific tasks.
Generating a synthetic dataset under DP is a generic task in that given the synthetic dataset, any task can be performed, and there is no need to modify existing non-private algorithms.  Compared to the ad-hoc methods, this approach may not achieve the optimal utility for the specific task.  
There are a number of previous studies focus on generating synthetic dataset in a differentially private manner.
We classify them into three categoreis: graphical model based methods, game based methods and deep generative model based methods.


\mypara{Graphical Model Based Methods}
The main idea is to estimate a graphical model that approximates the distribution of the original dataset in a differentially private way.
\privbayes~\cite{zhang2017privbayes} and \bsg~(the initials of the authors' last names)~\cite{bindschaedler2017plausible} approximate the data distribution using Bayesian Network.
These methods, however, need to call Exponential Mechanism~\cite{zhang2017privbayes} or Laplace Mechanism~\cite{bindschaedler2017plausible} many times, making the network structure inaccurate when the privacy budget is limited; and the overall utility is sensitive to the quality of the initial selected node.

\pgm~\cite{mckenna2019graphical} and \jtree~\cite{chen2015differentially} utilize Markov Random Field to approximate the data distribution.
\pgm takes as input a set of predefined low-dimensional marginals, and estimates a Markov Random Field that best matches these marginals.
\jtree first estimates a dependency graph by setting a threshold to the mutual information of pairwise attributes, and then obtains the Markov Random Field by transforming the dependency graph into a junction tree.
\pgm do not provide marginal selection method in the paper~\cite{mckenna2019graphical}.
\jtree proposes to use SVT to select marginals; however, Lyu \etal~\cite{lyu2016understanding} point out that JTree utilizes SVT in an incorrect way and violates DP.



\mypara{Game Based Methods}
There are works that formulate the dataset synthesis problem as a zero-sum game~\cite{hardt2012simple,gaboardi2014dual,vietrinew}.
Assume there are two players, data player and query player.
MWEM~\cite{hardt2012simple} method solves the game by having the data player use a no-regret learning algorithm, and the query player repeatedly best responds.
Dual Query~\cite{gaboardi2014dual} switches the role of the two players.
Concretely, the data player in MWEM maintains a distribution over the whole data domain, and query player repeatedly use exponential mechanism to select a query that have the worse performance from a workload of queries to update data player's distribution.
The main limitation of MWEM is that when the dataset domain is large (from $3 \cdot 10^{39}$ to $5 \cdot 10^{162}$ in our experiments), maintaining the full distribution is infeasible.
\todo{What are domain sizes in the competition.}
\zzk{$6.7 \times 10^{170}$.}

In contrast, the query player in Dual Query maintains a distribution over all queries.
The query player each time samples a set of queries from the workload, and the data player generates a record that minimizes the error of these queries.  
Detailed comparison with this method has been conducted in \cite{}. 
The shortcoming is that generating each record would consume a portion of privacy budget; thus one cannot generate sufficient records
 as discussed in Section~\ref{sec:exp}.
Moreover, both methods require a workload of queries in advance, and the generated dataset is guaranteed to be similar to the original dataset with respect to the query class.
This makes MWEM and Dual Query incapable of handling arbitrary kinds of tasks with satisfied accuracy.



\mypara{Deep Generative Model Based Methods}
Another approach is to train a deep generative model satisfying differential privacy, and use the deep generative model to generate a synthetic dataset.
The most commonly used deep generative model is the Generative Adversarial Network (GAN), and there are multiple studies focus on training GAN in a differentially private way~\cite{zhang2018differentially,beaulieu2019privacy,abay2018privacy,frigerio2019differentially,tantipongpipat2019differentially}.
The main idea is to utilize the DP-SGD framework~\cite{abadi2016deep} to add noise in the optimization procedure (i.e., stochastic gradient descent).
However, the preliminary application of GAN is to generate images.
Thus, the objective of GAN is to generate data records that look authentic, instead of approximating the original distribution, applying the GAN model to the current problem cannot generate a synthetic dataset with enough variations.
In the NIST challenge~\cite{nist-challenge}, there are two teams adapting the GAN-based method to synthesize high-dimensional data, while their scores are much lower than \pgm and \privbayes.
Thus, we do not compare this line of methods in our experiments.




